TWOLAR: a TWO-step LLM-Augmented distillation method for passage Reranking

In this paper, we present TWOLAR: a two-stage pipeline for passage reranking based on the distillation of knowledge from Large Language Models (LLM). TWOLAR introduces a new scoring strategy and a distillation process consisting in the creation of a novel and diverse training dataset. The dataset consists of 20K queries, each associated with a set of documents retrieved via four distinct retrieval methods to ensure diversity, and then reranked by exploiting the zero-shot reranking capabilities of an LLM. Our ablation studies demonstrate the contribution of each new component we introduced. Our experimental results show that TWOLAR significantly enhances the document reranking ability of the underlying model, matching and in some cases even outperforming state-of-the-art models with three orders of magnitude more parameters on the TREC-DL test sets and the zero-shot evaluation benchmark BEIR. To facilitate future work we release our data set, finetuned models, and code.

==> paper/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htb]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.5cm}
\centering
\scriptsize
\caption{We perform ablation studies on the eight smallest datasets in BEIR benchmark. The reported scores are nDCG@10. In comparing our scoring strategy against the RankT5 scoring strategy, the statistical tests yielded a p-value of \( p = \text{0.268} \). *COV: TREC-COVID, SCI: SciFact, NFC: NFCorpus, TOU: Tóuche-2020, DBP: DBPedia, ROB: Robust04, SIG: Signal-1M, NEW: TREC-NEWS. }
\label{table:ablation}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc|c}
\begin{tabular}{l|P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}|P{1cm}}
\hline \hline
% \multicolumn{1}{l|}{} & TREC-COVID & SciFact & NFCorpus & Tóuche-2020 & DBPedia & Robust04 & Signal-1M & \multicolumn{1}{l|}{TREC-NEWS} & avg nDCG@10 \\ \hline \hline

 & COV & SCI & NFC & TOU & DBP & ROB & SIG & NEW & avg \\ 
 \hline \hline

Score Strategy & \multicolumn{9}{c}{effectiveness of score strategy - 19K train samples}                                            \\ \hline
Difference & 74.0     & 67.9     & \textbf{31.9} & \textbf{35.7} & \textbf{38.8} & \textbf{47.4} & 32.5     & \textbf{43.7} & \textbf{46.5} \\
RankT5   & \textbf{74.1} & \textbf{69.2} & 31.5     & 32.2     & 36.2     & 47.0     & \textbf{34.1} & 41.2     &     45.7 \\ \hline \hline
\# documents & \multicolumn{9}{c}{effectiveness of amount of documents - 19K train samples}                                       \\ \hline
30         & \textbf{74.0} &     67.9 &     31.9 & \textbf{35.7} & \textbf{38.8} &     47.4 & \textbf{32.5} & \textbf{43.7} & \textbf{46.5} \\
20         &     73.0 & \textbf{69.8} & \textbf{32.5} &     31.7 &     37.9 & \textbf{47.5} &     31.9 &     40.8 &     46.3 \\
10         &     72.3 &     65.6 &     29.6 &     28.4 &     34.2 &     43.2 &     30.4 &     37.9 &     42.7 \\ \hline \hline
Not used source & \multicolumn{9}{c}{effectiveness of first source of supervision - $\sim$14K train samples}                         \\ \hline
- BM25     &     72.7 &     70.3 &     31.8 &     31.8 &     37.7 &     47.0 &     31.9 &     41.5 &     45.6 \\
- SPLADE   &     73.9 & \textbf{70.9} & \textbf{33.6} &     32.7 & \textbf{38.6} & \textbf{48.8} &     32.4 &     42.5 & \textbf{46.3} \\
- DRAGON   & \textbf{74.0} &     67.7 &     32.9 & \textbf{33.9} &     37.6 &     47.7 & \textbf{33.1} &     43.2 &     46.2 \\
- monoT5   &     73.9 &     69.4 &     31.8 &     33.0 &     36.3 &     46.6 &     32.5 & \textbf{43.6} &     45.9 \\ \hline \hline
Type of query & \multicolumn{9}{c}{effectiveness of type of query - 9.5K train samples}                                            \\ \hline
Mixed      & \textbf{75.5} &     67.3 &     30.4 & \textbf{34.0} &     37.2 & \textbf{46.2} & \textbf{31.8} &     41.6 & \textbf{45.5} \\
Sentence   &     67.2 & \textbf{67.9} & \textbf{31.4} &     32.7 &     32.2 &     44.8 &     31.7 &     39.7 &     43.4 \\
docT5query &     74.6 &     59.4 &     31.2 &     33.4 & \textbf{37.8} &     44.9 &     28.1 & \textbf{44.0} &     44.2 \\ \hline \hline
\end{tabular}%
% }
\vspace{-0.5cm}
\end{table}

==> paper/beir-1000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[hbt]
\centering
\caption{Results on the BEIR Benchmark by reranking the top 1000 BM25 retrieved documents. The best model is highlighted in boldface, and the second best is underlined for each dataset. All results, apart from TWOLAR-xl, are from~\cite{inparsv2}.}
\scriptsize
\label{table:beir-1000}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l||c|cccc}
\hline \hline
 & BM25 & monoT5-3B & InPars-v2 & RankT5 & TWOLAR-xl \\ \hline
 \multicolumn{6}{c}{nDCG@10} \\ \hline
TREC-COVID &
  59.5 &
  80.1 &
  {\bf 84.6} &
  82.3 &
  {\ul 84.3} \\ %\cline{1-1}
NFCorpus &
  32.2 &
  38.3 &
  {\ul 38.5} &
  {\bf 39.9} &
  37.3 \\ %\cline{1-1}
FiQA-2018 &
  23.6 &
  {\bf 50.9} &
  {\ul 50.9} &
  49.3 &
  45.2 \\ %\cline{1-1}
ArguAna &
  30.0 &
  {\ul 37.9} &
  36.9 &
  {\bf 40.6} &
  32.7 \\ %\cline{1-1}
Tóuche-2020 &
  {\ul 44.2} &
  30.9 &
  29.1 &
  {\bf 48.6} &
  35.9 \\ %\cline{1-1}
Quora &
  78.9 &
  83.5 &
  {\ul 84.5} &
  81.9 &
  {\bf 87.3} \\ %\cline{1-1}
SCIDOCS &
  14.9 &
  19.7 &
  {\bf 20.8} &
  19.1 &
  {\ul 20.3} \\ %\cline{1-1}
SciFact &
  67.9 &
  {\bf 77.4} &
  {\ul 77.4} &
  76.0 &
  76.8 \\ %\cline{1-1}
NQ &
  30.6 &
  62.5 &
  63.8 &
  {\bf 64.7} &
  {\ul 64.2} \\ %\cline{1-1}
HotpotQA &
  63.3 &
  76.0 &
  {\ul 79.1} &
  75.3 &
  {\bf 79.5} \\ %\cline{1-1}
DBPedia &
  31.8 &
  47.2 &
  {\ul 49.8} &
  45.9 &
  {\bf 52.0} \\ %\cline{1-1}
FEVER &
  65.1 &
  84.8 &
  {\bf 87.2} &
  84.8 &
  {\ul 86.7} \\ %\cline{1-1}
Climate-FEVER &
  16.5 &
  {\ul 28.8} &
  {\bf 32.3} &
  27.5 &
  27.8 \\ %\cline{1-1}
CQADupStack &
  30.2 &
  {\bf 44.9} &
  {\ul 44.8} &
  - &
  43.8 \\ %\cline{1-1}
Robust04 &
  40.8 &
  61.5 &
  {\ul 63.2} &
  - &
  {\bf 64.2} \\ %\cline{1-1}
Signal-1M &
  {\bf 33.1} &
  30.2 &
  30.8 &
  {\ul 31.9} &
  31.5 \\ %\cline{1-1}
BioASQ &
  52.3 &
  56.6 &
  {\bf 59.5} &
  {\ul 57.9} &
  56.0 \\ %\cline{1-1}
TREC-NEWS &
  39.5 &
  47.7 &
  {\ul 49.0} &
  - &
  {\bf 53.2} \\ \hline
  \multicolumn{6}{c}{avg nDCG@10} \\ \hline
 BEIR 18 &
  41.9 &
  53.3 &
  {\bf 54.5} &
  - &
  {\ul 54.4} \\ 
 BEIR 15 &
  42.9 &
  53.7 &
  {\ul 54.9} &
  {\bf 55.0} &
  54.5 \\ \hline \hline

\end{tabular}%
% }

\vspace{-0.5cm}
\end{table}

==> paper/beir_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[htb]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{0.25cm}
\caption{Results on the BEIR Benchmark by reranking the top 100 documents with different retrievers. Best model is in boldface and second best is underlined for each dataset. Evaluation for InPars on CQADupStack is missing due to its unavailability on the Hugging Face hub. We computed statistical tests comparing our biggest model against the baselines. The results revealed no significant difference compared to InPars \( (p = 0.477) \), but indicated significant improvements over MonoT5-3B \( (p = 4.20 \times 10^{-4}) \) and RankGPT-Deberta \( (p = 2.82 \times 10^{-13}) \). It's noteworthy that while our model operates in a zero-shot manner, the InPars models have been fine-tuned for each BEIR dataset.}
\label{table:beir_result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l||c|ccccc||c|ccccc||c|ccccc}
\hline \hline
\multicolumn{1}{c||}{Retriever} &
  \multicolumn{6}{c||}{BM25} &
  \multicolumn{6}{c||}{SPLADE} &
  \multicolumn{6}{c}{DRAGON} \\ \hline
\multicolumn{1}{c||}{\rotatebox{280}{Reranker}} &
  - &
  \rotatebox{280}{MonoT5-3B} &
  \rotatebox{280}{InPars} &
  \rotatebox{280}{RankGPT-Deberta  } &
  \rotatebox{280}{TWOLAR-xl} &
  \multicolumn{1}{l||}{\rotatebox{280}{TWOLAR-large}} &
  - &
  \rotatebox{280}{MonoT5-3B} &
  \rotatebox{280}{InPars} &
  \rotatebox{280}{RankGPT-Deberta} &
  \rotatebox{280}{TWOLAR-xl} &
  \multicolumn{1}{l||}{\rotatebox{280}{{TWOLAR-large}}} &
  - &
  \rotatebox{280}{MonoT5-3B} &
  \rotatebox{280}{InPars} &
  \rotatebox{280}{RankGPT-Deberta} &
  \rotatebox{280}{TWOLAR-xl} & 
  \rotatebox{280}{TWOLAR-large} \\ \hline
  \multicolumn{19}{c}{nDCG@10} \\ \hline
TREC-COVID &
  59.5 &
  79.8 &
  82.5 &
  79.4 &
  82.7 & 
  84.3 & %%
  72.8 &
  82.9 &
  85.7 &
  80.1 & 
  85.2 &
  {\bf 86.9} & %%
  75.8 &
  82.8 &
  84.8 &
  82.6 &
  84.6 &
  {\ul 86.8} \\ %\cline{1-1}
NFCorpus &
  32.2 & 
  37.4 &
  35.0 &
  33.3 &
  36.6 &
  35.7 & %%
  34.8 &
  39.2 &
  38.8 &
  33.2 &
  37.3 &
  35.5 & %%
  33.9 &
  {\bf 39.7} &
  {\ul 39.3} &
  33.2 &
  37.9 &
  35.7 \\ %\cline{1-1}
FiQA-2018 &
  23.6 &
  46.1 &
  46.2 &
  32.7 &
  41.9 &
  41.1 & %%
  34.8 &
  50.0 &
  50.0 &
  33.7 &
  44.8 &
  43.8 & %%
  35.7 &
  {\bf 51.2} &
  {\ul 50.9} &
  43.1 &
  45.3 &
  44.8 \\ %\cline{1-1}
ArguAna &
  30.0 &
  33.4 &
  32.8 &
  21.1 &
  32.9 &
  34.7 & %%
  38.8 &
  31.7 &
  31.2 &
  18.6 &
  32.9 &
  34.6 & %%
  {\bf 46.9} &
  41.5 &
  40.9 &
  25.7 &
  42.8 &
  {\ul 45.5} \\ %\cline{1-1}
Tóuche-2020 &
  \textbf{44.2} &
  31.6 &
  29.6 &
  37.7 &
  37.1 &
  33.4 & %%
  24.6 &
  29.8 &
  28.7 &
  36.4 &
  35.2 &
  30.4 & %%
  26.3 &
  30.6 &
  29.4 &
  {\ul 38.2} &
  36.0 & 
  31.5 \\ %\cline{1-1}
Quora &
  78.9 &
  84.1 &
  84.8 &
  78.8 &
  87.2 &
  86.0 & %%
  83.5 &
  84.3 &
  85.1 &
  80.3 &
  {\ul 87.4} &
  86.0 & %%
  {\bf 87.5} &
  83.5 &
  84.4 &
  78.7 &
  87.2 & 
  85.7 \\ %\cline{1-1}
SCIDOCS &
  14.9 &
  19.0 &
  19.2 &
  16.1 &
  19.5 &
  18.3 & %% 
  15.9 &
  19.9 &
  {\bf 20.9} &
  16.4 &
  20.2 &
  18.8 & %%
  15.9 &
  19.8 &
  {\ul 20.7} &
  16.4 &
  20.2 & 
  18.8 \\ %\cline{1-1}
SciFact &
  67.9 &
  {\ul 76.4} &
  73.5 &
  70.5 &
  {\bf 76.5} &
  75.6 & %% 
  70.2 &
  {\ul 76.4} &
  76.0 &
  69.1 &
  75.6 &
  74.7 & %%
  67.8 &
  76.0 &
  75.7 &
  69.4 &
  75.6 &
  74.7 \\ %\cline{1-1}
NQ &
  30.6 &
  56.8 &
  57.8 &
  46.1 &
  58.0 &
  57.7 & %%
  53.7 &
  65.9 &
  66.4 &
  50.6 &
  {\ul 66.8} &
  65.8 & %%
  53.8 &
  65.1 &
  66.6 &
  50.6 &
  {\bf 66.9} &
  66.2 \\ %\cline{1-1}
HotpotQA &
  63.3 &
  74.2 &
  76.5 &
  69.9 &
  76.7 &
  75.9 & %%
  68.7 &
  74.1 &
  {\ul 77.1} &
  70.5 &
  {\bf 77.7} &
  76.4 & %%
  66.2 &
  72.9 &
  75.7 &
  69.8 &
  76.4 & 
  75.3 \\ %\cline{1-1}
DBPedia &
  31.8 &
  44.8 &
  44.0 &
  41.9 &
  48.0 &
  47.8 & %%
  43.6 &
  48.2 &
  51.1 &
  45.9 &
  {\bf 52.9} &
  51.6 & %%
  41.9 &
  47.2 &
  50.3 &
  44.9 &
  {\ul 52.1} &
  51.3 \\ %\cline{1-1}
FEVER &
  65.1 &
  83.2 &
  85.5 &
  80.2 &
  84.9 &
  83.4 & %%
  79.3 &
  85.0 &
  88.0 &
  81.8 &
  {\ul 87.5} &
  85.4 & %%
  78.0 &
  84.7 &
  {\bf 87.7} &
  81.7 &
  87.2 & 
  85.2 \\ %\cline{1-1}
Climate-FEVER &
  16.5 &
  27.4 &
  30.1 &
  24.2 &
  26.9 &
  26.1 & %%
  22.9 &
  28.7 &
  {\bf 32.8} &
  25.9 &
  28.9 &
  27.9 & %%
  22.7 &
  28.6 &
  {\ul 32.5} &
  25.9 &
  28.6 &
  27.4 \\ %\cline{1-1}
CQADupStack &
  30.2 &
  41.5 &
  - &
  34.7 &
  41.2 &
  40.6 & %%
  33.4 &
  43.7 &
  - &
  35.9 &
  43.6 &
  42.7 & %%
  35.4 &
  {\bf 44.4} &
  - &
  36.0 &
  {\ul 44.2} &
  43.4 \\ %\cline{1-1}
Robust04 &
  40.8 &
  56.6 &
  58.7 &
  52.8 &
  57.9 &
  58.3 & %%
  46.7 &
  62.1 &
  \textbf{64.3} &
  57.3 &
  64.9 &
  65.2 & %%
  48.1 &
  61.3 &
  {\ul 63.2} &
  56.6 &
  63.4 & 
  63.7 \\ %\cline{1-1}
Signal-1M &
  33.1 &
  32.2 &
  32.9 &
  {\ul 33.4} &
  \textbf{33.8} &
  33.9 & %% 
  30.0 &
  29.4 &
  30.3 &
  30.0 &
  30.1 &
  30.5 & %%
  30.0 &
  29.7 &
  30.4 &
  29.4 &
  30.2 &
  30.1 \\ %\cline{1-1}
BioASQ &
  52.3 &
  {\ul 57.2} &
  \textbf{59.8} &
  53.0 &
  56.2 &
  56.0 & %%
  49.7 &
  54.1 &
  57.2 &
  49.5 &
  54.6 &
  53.8 & %%
  43.4 &
  51.9 &
  54.4 &
  48.0 &
  51.9 &
  50.8 \\ %\cline{1-1}
TREC-NEWS &
  39.5 &
  48.5 &
  49.8 &
  51.8 &
  52.7 &
  50.8 & %%
  41.5 &
  50.0 &
  50.9 &
  {\ul 53.4} &
  53.3 &
  50.7 & %%
  44.4 &
  49.5 &
  50.8 &
  52.1 &
  {\bf 53.8} &
  50.0 \\ \hline
  \multicolumn{19}{c}{avg nDCG@10} \\ \hline
\multicolumn{1}{l||}{BEIR 18} &
  41.9 &
  51.7 &
  - &
  47.6 &
  52.8 &
  52.2 & %%
  46.9 &
  53.0 &
  - &
  48.3 &
  {\ul 54.4} &
  53.4 & %%
  47.4 &
  53.4 &
  - &
  48.5 &
  {\bf 54.7} &
  53.7 \\ 
\multicolumn{1}{l||}{BEIR 17} &
  42.6 &
  52.3 &
  52.9 &
  48.4 &
  53.5 &
  52.9 & %%
  47.8 &
  53.5 &
  55.0 &
  49.0 &
  55.0 &
  54.0 & %%
  48.1 &
  53.9 &
  {\ul 55.2} &
  49.2 &
  {\bf 55.3} &
  54.3 \\ \hline \hline

\end{tabular}%
}
\vspace{-0.5cm}
\end{table}

==> paper/intersection_source.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htb]
    \setlength{\abovecaptionskip}{-0.5cm}
\setlength{\belowcaptionskip}{0.25cm}
\caption{Average intersection rate between each pair of sources. The upper triangular part of the table represents the intersection rate for cropped sentences and the lower triangular part represents the intersection rate for docT5query-generated queries.}
\label{table:intersection_sources}
\centering
\scriptsize
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc}
\hline \hline
doct5query \textbackslash \ cropped sentence (\%) & BM25             & SPLADE           & DRAGON           & monoT5           \\ \hline
BM25                               & \textbackslash{} & 20.0             & 29.0             & 49.8             \\
SPLADE                             & 17.8             & \textbackslash{} & 35.8             & 26.0             \\
DRAGON                             & 25.0             & 41.0             & \textbackslash{} & 38.4             \\
monoT5                             & 46.4             & 27.2             & 38.5             & \textbackslash{} \\ \hline \hline
\end{tabular}%
% }
\vspace{-.5cm}
\end{table}


==> paper/supervised_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[htb]
\setlength{\abovecaptionskip}{-0.cm}
\setlength{\belowcaptionskip}{0.5cm}
\caption{Results on TREC-DL2019 and TREC-DL2020 datasets by reranking top 100 documents retrieved by BM25. The column titled `\#Calls' indicates the exact number of inference times of LLM when reranking the top 100 documents. The `Input Size' column uses the notation $|q|+n|d|$: $|q|$ represents one query and $n|d|$ indicates the number of documents included. For instance, $|q|+20|d|$ signifies an input of one query with $20$ documents. Best model is highlighted in boldface and the second best is underlined for each metric. All the reported results apart from the LLM distillation Methods are taken from the original papers.}
\label{table:supervised_res}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllcccccc}
\hline \hline
\multicolumn{1}{l|}{Method}         & \multicolumn{1}{l|}{LLM}           & \multicolumn{1}{l|}{Size}           & \multicolumn{1}{l|}{\#Calls} & \multicolumn{1}{l|}{Input Size}           & \multicolumn{3}{c|}{TREC-DL2019}                & \multicolumn{3}{c}{TREC-DL2020} \\ \hline
 
  \multicolumn{5}{l|}{} &
  \multicolumn{1}{c}{nDCG@1} &
  \multicolumn{1}{c}{nDCG@5} &
  \multicolumn{1}{c|}{nDCG@10} &
  \multicolumn{1}{c}{nDCG@1} &
  \multicolumn{1}{c}{nDCG@5} &
  \multicolumn{1}{c}{nDCG@10} \\ \hline
\multicolumn{1}{l|}{BM25}           & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-}& \multicolumn{1}{l|}{-}& \multicolumn{1}{l|}{-}            & 54.26       & 52.78 & \multicolumn{1}{c|}{50.58} & 57.72         & 50.67   & 47.96  \\ \hline
\multicolumn{11}{c}{Supervised Methods} \\ \hline
\multicolumn{1}{l|}{monoBERT}       & \multicolumn{1}{l|}{BERT}     & \multicolumn{1}{l|}{340M} & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{$~|q|+|d|$}    & 79.07       & 73.25 & \multicolumn{1}{c|}{70.50} & 78.70         & 70.74   & 67.28  \\
\multicolumn{1}{l|}{monoT5}         & \multicolumn{1}{l|}{T5-xl}    & \multicolumn{1}{l|}{3B} & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{$~|q|+|d|$}    & 79.07       & 73.74 & \multicolumn{1}{c|}{71.83} & 80.25         & 72.32   & 68.89  \\
\multicolumn{1}{l|}{RankT5}         & \multicolumn{1}{l|}{T5-xl}    & \multicolumn{1}{l|}{3B} & \multicolumn{1}{l|}{100}  & \multicolumn{1}{l|}{$~|q|+|d|$}   & 77.38       & 73.94 & \multicolumn{1}{c|}{71.22} & {\ul 80.86}         & 72.99   & 69.49  \\ \hline
\multicolumn{11}{c}{LLM distillation Methods}   \\ \hline
\multicolumn{1}{l|}{RankGPT}       & \multicolumn{1}{l|}{DeBertaV2}  & \multicolumn{1}{l|}{184M} & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{$~|q|+|d|$} & 78.68       & 69.77 & \multicolumn{1}{c|}{66.56} &  59.26  &  59.83   & 59.43  \\
\multicolumn{1}{l|}{TWOLAR-large}       & \multicolumn{1}{l|}{Flan-T5-large}  & \multicolumn{1}{l|}{783M} & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{$~|q|+|d|$} & 79.84       & 75.94 & \multicolumn{1}{c|}{72.82} & 79.94   & 71.35   & 67.61  \\ 
\multicolumn{1}{l|}{TWOLAR-xl}       & \multicolumn{1}{l|}{Flan-T5-xl}  & \multicolumn{1}{l|}{3B} & \multicolumn{1}{l|}{100} & \multicolumn{1}{l|}{$~|q|+|d|$} & 78.29       & {\ul 76.71} & \multicolumn{1}{c|}{{\ul 73.51}} & 80.25   & 73.73   & \bf 70.84  \\ \hline
\multicolumn{11}{c}{Zero-shot LLM Methods}  \\ \hline
\multicolumn{1}{l|}{RankGPT}        & \multicolumn{1}{l|}{gpt-3.5-turbo} & \multicolumn{1}{l|}{154B$^\ast$} & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{$~|q|+20|d|$} & {\ul 82.17} & 71.15 & \multicolumn{1}{c|}{65.80} & 79.32         & 66.76   & 62.91  \\
\multicolumn{1}{l|}{RankGPT} &
  \multicolumn{1}{l|}{gpt-4} & \multicolumn{1}{l|}{1T$^\ast$} & \multicolumn{1}{l|}{2$^\dagger$} & \multicolumn{1}{l|}{$~|q|+20|d|$} &
  \textbf{82.56} &
  \textbf{79.16} &
  \multicolumn{1}{c|}{\textbf{75.59}} &
  78.40 &
  {\ul 74.11} &
  {\ul 70.56} \\
\multicolumn{1}{l|}{PRP-Sliding-10} & \multicolumn{1}{l|}{Flan-T5-xl} & \multicolumn{1}{l|}{3B} & \multicolumn{1}{l|}{990}  & \multicolumn{1}{l|}{$~|q|+2|d|$} & 75.58       & 71.23 & \multicolumn{1}{c|}{68.66} & 75.62         & 69.00   & 66.59  \\
\multicolumn{1}{l|}{PRP-Sliding-10} & \multicolumn{1}{l|}{Flan-T5-xxl} & \multicolumn{1}{l|}{11B} & \multicolumn{1}{l|}{990} & \multicolumn{1}{l|}{$~|q|+2|d|$} & 64.73       & 69.49 & \multicolumn{1}{c|}{67.00} & 75.00         & 70.76   & 67.35  \\
\multicolumn{1}{l|}{PRP-Sliding-10} &
  \multicolumn{1}{l|}{Flan-UL2} & \multicolumn{1}{l|}{20B} & \multicolumn{1}{l|}{990} & \multicolumn{1}{l|}{$~|q|+2|d|$}&
  78.29 &
  75.49 &
  \multicolumn{1}{c|}{72.65} &
  \textbf{85.80} &
  \textbf{75.35} & 
  70.46 \\ \hline \hline 
  \multicolumn{11}{l}{$^\ast$ OpenAI has not publicly released the amount of parameters and the numbers are based on public estimates \cite{gpt3.5vsgpt4} \cite{gpt4-review-opp}.} \\
  \multicolumn{11}{l}{$^\dagger$ In \cite{rankgpt}, gpt-4 reranks the top-30 passages reranked by gpt-3.5-turbo.}
 
\end{tabular}%
}
\vspace{-0.5cm}
\end{table}
